Identifying First-person Camera Wearers in Third-person Videos

We consider scenarios in which we wish to perform joint scene understanding, object tracking, activity recognition, and other tasks in environments in which multiple people are wearing body-worn cameras while a third-person static camera also captures the scene. To do this, we need to establish person-level correspondences across first- and third-person videos, which is challenging because the camera wearer is not visible from his/her own egocentric video, preventing the use of direct feature matching. In this paper, we propose a new semi-Siamese Convolutional Neural Network architecture to address this novel challenge. We formulate the problem as learning a joint embedding space for first- and third-person videos that considers both spatial- and motion-domain cues. A new triplet loss function is designed to minimize the distance between correct first- and third-person matches while maximizing the distance between incorrect ones. This end-to-end approach performs significantly better than several baselines, in part by learning the first- and third-person features optimized for matching jointly with the distance measure itself.

==> metric.tex <==
\section{Metric learning for first-person and third-person video with Siamese networks}
The purpose of this paper is to learn a proper distance metric which gets a measure of distance between the camera wearers of egocentric videos and those identities appear in third-person videos. The expectation is the actual camera wearer of first-person video and the bounding box of this person in third-person video should have a closer distance, while the other persons in third-person video should have larger distances.
Siamese networks, as well as triplet Siamese networks are now used to learn this metric.
In Siamese networks, we will give a pair which includes first-person frame and one bounding box of a person in third-person frame . If the camera wearer of first-person video is identical to the person in bounding box, this pair gets true label; otherwise this pair gets a false label since the person in bounding box cannot correspond to first-person video. 
In triplet Siamese networks, we input first-person video, the actual person's representation ( either masked frame in spatial network or cropped optical flow in temporal network), as well as a randomly selected non-relevant person's representation in third-person video. By feeding both true pairs and false pairs and calculating the distances between true pairs and distances between false pairs, we can use triplet loss function as described in \ref{sect:lossfunction} to explicitly enlarge the difference of the two distances.
